Exploring the Ecosystem of DNS HTTPS Resource Records: An End-to-End Perspective

The DNS HTTPS resource record is a new DNS record type designed for the delivery of configuration information and parameters required to initiate connections to HTTPS network services. In addition, it is a key enabler for TLS Encrypted ClientHello (ECH) by providing the cryptographic keying material needed to encrypt the initial exchange. To understand the adoption of this new DNS HTTPS record, we perform a longitudinal study on the server-side deployment of DNS HTTPS for Tranco top million domains, as well as an analysis of the client-side support for DNS HTTPS through snapshots from major browsers. To the best of our knowledge, our work is the first longitudinal study on DNS HTTPS server deployment, and the first known study on client-side support for DNS HTTPS. Despite the rapidly growing trend of DNS HTTPS adoption, our study highlights challenges and concerns in the deployment by both servers and clients, such as the complexity in properly maintaining HTTPS records and connection failure in browsers when the HTTPS record is not properly configured.

==> sections/6_security.tex <==
\section{Discussion}
\label{sec:discussion}

%\ys{fill in the end, potential discussion section}

%\noindent Potential topics:
%\begin{itemize}
%    \item Misconfigured server
%    \item Incorrectly-formatted resource record
%    \item ECH-related?
%    \item RRSIG HTTPS RR-related?
%    \item ...
%\end{itemize}

\paragraph{Measurement Coverage.}
In this research, we leverage the Tranco list to assess the deployment of \https records.
This approach allows us to concentrate on exploring how \https records are deployed and managed among popular domains.
However, this methodology restricts our ability to investigate \https record deployment among other domains not listed in the Tranco list (e.g., domains that are less popular).
Therefore, in our future work, we aim to expand our measurement scope to encompass the entire domain name space.

\hmlee{can be omitted.}

\paragraph{Automation Tool for \https record Management.}
As highlighted earlier, managing \https records presents complexities due to their DNS-based nature.
Inconsistency issues can arise when domains manage their \https records without accounting for DNS caching effects, which specifically can lead to issues with IP hints (i.e., \ipfh/\ipsh) or ECH configurations (i.e., \ech).
A notable concern is a mismatch between the ECH key specified in \ech parameters and the actual key used by the server (e.g., TLS server).%, which could hinder the encryption of the TLS \chello message.

\texttt{Let's Encrypt} has significantly reduced the barriers to HTTPS adoption by automating the certificate issuance process through \texttt{ACME} and \texttt{Certbot}~\cite{aas2019let,tiefenau2019usability}, demonstrating the potential benefits of automation in managing web security features.
Given this context, we believe that an automation tool designed for \https record management could address these DNS cache-related challenges.
Consequently, our future work will also focus on developing such a tool, equipped with features to automatically update IP hints and ECH configurations in \https records, thereby enhancing the overall security and reliability of \https record ecosystem.


==> tables/apx_ipmismatch_detail.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{Date} & \textbf{Apex} & \textbf{\#IPs in A) & \texttt{\#IPs in A reachable} & \textbf{\#IPs in \ipsh} & \begin{tabular}[c]{@{}l@{}}\#IPs in IPv4hint\\    \\ connected\end{tabular} & \#IPs in AAAA & \begin{tabular}[c]{@{}l@{}}\#IPs in AAAA\\    \\ Connected\end{tabular} & \#IPs in IPv6hint & \begin{tabular}[c]{@{}l@{}}\#IPs in IPv6hint\\    \\ connected\end{tabular} \\ \hline
2024-01-25 & filterchy.cfd & 1 & 0 & 2 & 0 & 1 & 0 & 2 & 0 \\ \hline
2024-01-26 & spurl.net & 1 & 0 & 2 & 2 & 0 & 0 & 0 & 0 \\ \hline
2024-01-26 & filterchy.cfd & 1 & 0 & 2 & 0 & 1 & 0 & 2 & 0 \\ \hline
2024-01-27 & filterchy.cfd & 1 & 0 & 2 & 0 & 1 & 0 & 2 & 0 \\ \hline
2024-01-28 & zuka168.com & 1 & 0 & 2 & 2 & 0 & 0 & 0 & 0 \\ \hline
2024-01-28 & evcobhi.cn & 1 & 0 & 2 & 2 & 0 & 0 & 0 & 0 \\ \hline
2024-01-28 & fvzhelh.cn & 1 & 0 & 2 & 2 & 0 & 0 & 0 & 0 \\ \hline
2024-01-28 & fnnlvdx.cn & 1 & 0 & 2 & 2 & 0 & 0 & 0 & 0 \\ \hline
2024-01-28 & filterchy.cfd & 1 & 0 & 2 & 0 & 1 & 0 & 2 & 0 \\ \hline
2024-01-28 & gyecujy.cn & 1 & 0 & 2 & 2 & 0 & 0 & 0 & 0 \\ \hline
2024-01-28 & dpjtmtd.cn & 1 & 0 & 2 & 2 & 0 & 0 & 0 & 0 \\ \hline
2024-01-28 & drvpzwl.cn & 1 & 0 & 2 & 2 & 0 & 0 & 0 & 0 \\ \hline
2024-01-28 & grslww.cn & 1 & 0 & 2 & 2 & 0 & 0 & 0 & 0 \\ \hline
2024-01-29 & crl.com & 2 & 1 & 2 & 0 & 0 & 0 & 0 & 0 \\ \hline
2024-01-29 & mln-free.com & 1 & 0 & 2 & 2 & 0 & 0 & 0 & 0 \\ \hline
2024-01-31 & crl.com & 2 & 1 & 2 & 0 & 0 & 0 & 0 & 0 \\ \hline
\end{tabular}
\end{table}

==> tables/tab-alpn-analysis.tex <==

\begin{table}[!htbp]
\resizebox{\columnwidth}{!}{%
\centering
\begin{tabular}{cc|c|c|c}
\multicolumn{2}{c|}{\multirow{4}{*}{\bf Protocols}} & \multicolumn{3}{c}{\textbf{\% of Apex Domains with}} \\
%\cline{2-4}
 & & \multicolumn{2}{c|}{\bf \cf NS} & \multirow{3}{*}{\shortstack[c]{\bf Non \\ \bf -\cf \\ \bf NS}} \\ \cline{3-4} 
 & & \multirow{2}{*}{\shortstack[c]{\bf Default \\ \bf conf}}  & \multirow{2}{*}{\shortstack[c]{\bf Custom \\ \bf conf}} &   \\ 
 & & & & \\ \hline
\multicolumn{2}{c|}{\textbf{\textcolor{red}{HTTP/2}}} &  99.66  &   & a \\ 
\multicolumn{2}{c|}{\textbf{\textcolor{red}{HTTP/3}}}  & 79.02  &  & b \\ 
\multirow{2}{*}{\shortstack[c|]{\bf HTTP/\\\bf 3-29}} & \multicolumn{1}{|c|}{$<$ May 31} & 77.43  & c & c \\
& \multicolumn{1}{|c|}{$\geq$ May 31} & $<$ 0.01  & d  & d \\ 
\multicolumn{2}{c|}{\textbf{HTTP/3-27}}  & $<$ 0.01  & d & d  \\ 
\multicolumn{2}{c|}{\textbf{HTTP/1.1}}  & $<$ 0.01 & e & e \\ 
\end{tabular}
}
\caption{Application layer protocols specified in the \alpn parameter (of \https records) for overlapping domains, on a daily average. Protocols highlighted in red are those in \cf's default \https record configuration. \hy{Todo - fill numbers}}
\label{tab:alpn-by-conf}
\end{table}

==> tables/tab-dnssec_val_results.tex <==
\begin{table}[t!]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{c||r||c|c}
    \multirow{2}{*}{\bf Category} & \multicolumn{3}{c}{\bf Domains} \\
    & \bf Signed & \bf \texttt{Secure} & \bf \texttt{Insecure}  \\% & \multirow{2}{*}{\bf Bogus} \\
    \hline
    \multicolumn{1}{l||}{without \https RR} & 46,850 & 35,688 (76.2\%) & 11,121 (23.7\%) \\
    \hline
    \multicolumn{1}{l||}{with \https RR} & 16,849 & 8,527 (50.6\%) & 8,322 (49.4\%)\\ % & 0 \\

    \multicolumn{1}{l||}{- \cf} & 16,784 & 8,471 (50.5\%) & 8,313 (49.5\%)\\ % & 0 \\
    \multicolumn{1}{l||}{- Non-\cf} & 64 & 55 (85.9\%) & 9 (14.1\%)\\ % & 0 \\
    \end{tabular}
    }
    \caption{The number of domains with signed records and their DNSSEC validation results, as of January 2nd, 2024. Domains with \https records are broken down based on their name servers (i.e., \cf or Non-\cf).
    We validate the DNSSEC chain of \https records if a domain published \https records, and the DNSSEC chain of \dnskey records for a domain without \https records. Note that \bogus validation results are omitted as there are no \bogus \https records.}
    \label{tab:dnssec-stats}
\vspace{-4mm}
\end{table}

==> tables/tab-nameservers.tex <==
\begin{table}[!ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ c|cc|cc }
      \multirow{3}{*}{\shortstack[c]{\bf Name Server (NS) \\ \bf Category}} & \multicolumn{2}{c|}{\bf Dynamic} & \multicolumn{2}{c}{\multirow{2}{*}{\bf Overlapping}} \\
      & \multicolumn{2}{c|}{\bf Tranco top 1M} & & \\
      & Mean & Std.& Mean & Std. \\
     \hline
     \makecell[l]{Full \textit{Cloudflare} NS} & 98.11 & 9.52 & 98.11 & 9.67\\    
     %\makecell[l]{Partial \textit{Cloudflare} NS} & 0.003 & 0.001 & 0.004 & 0.001 \\     
     \makecell[l]{Non-\textit{Cloudflare} NS} & 1.88 & 9.52 & 1.88 & 9.67 \\
\end{tabular}
}
\caption{The average and standard deviation of the percentage of apex domains served by either Cloudflare or non-Cloudflare name servers are shown. \hmlee{Hongying - how about this one? Partial cloudflare is negligible and not be used in further analysis, so we can just briefly mention it in the paragraph.}} 
\label{tab:nsinfoalldom2}
\end{table}
